U-Net v2: Rethinking the Skip Connections of U-Net for Medical Image Segmentation

In this paper, we introduce U-Net v2, a new robust and efficient U-Net variant for medical image segmentation. It aims to augment the infusion of semantic information into low-level features while simultaneously refining high-level features with finer details. For an input image, we begin by extracting multi-level features with a deep neural network encoder. Next, we enhance the feature map of each level by infusing semantic information from higher-level features and integrating finer details from lower-level features through Hadamard product. Our novel skip connections empower features of all the levels with enriched semantic characteristics and intricate details. The improved features are subsequently transmitted to the decoder for further processing and segmentation. Our method can be seamlessly integrated into any Encoder-Decoder network. We evaluate our method on several public medical image segmentation datasets for skin lesion segmentation and polyp segmentation, and the experimental results demonstrate the segmentation accuracy of our new method over state-of-the-art methods, while preserving memory and computational efficiency. Code is available at: https://github.com/yaoppeng/U-Net_v2

==> tables/polyp_1.tex <==
\begin{table*}[h]
\centering
\small
\begin{tabular}{c|cccccccccccc}

\multirow{2}{*}{Method} & \multicolumn{3}{c}{Kvasir-SEG} & \multicolumn{3}{c}{ClinicDB} & \multicolumn{3}{c}{ColonDB}\\

\cline{2-10}

& DSC (\%) & mIoU (\%)  & MAE & DSC (\%) &mIoU (\%)  & MAE & DSC (\%) & mIoU (\%) &  MAE \\

\hline 

U-Net~\cite{ronneberger2015u}  & 81.8 & 74.6 & 0.055 & 82.3 & 75.5 & 0.019 & 51.2 & 44.4 & 0.061 \\

UNet++~\cite{zhou2018unet++} & 82.1 & 74.3 & 0.048 & 79.4 & 72.9 & 0.022 & 48.3 & 41.0 & 0.064\\

PraNet~\cite{fan2020pranet} & 89.8 & 84.0 & 0.030 & 89.9 & 84.9 & 0.009 & 71.2 & 64.0 & 0.043 \\

SANet~\cite{wei2021shallow} & 90.4 & 84.7 & 0.028 & 91.6 & 85.9 & 0.012 & 75.3 & 67.0 & 0.043\\

Polyp-PVT~\cite{dong2021polyp} & 91.7 & 86.4 & 0.023 & 93.7 & 88.9 & \textbf{0.006} & 80.8 & 72.7 & 0.031\\

% U-Net (PVT)~\cite{ronneberger2015u} & 0.925 & 0.875 & 0.023 & 0.936 & 0.888 & 0.007 & 0.792 & 0.715 & 0.030 \\

% UNet++ (PVT)~\cite{zhou2018unet++} & 0.928 & 0.879 & 0.020 & 0.933 & 0.885 & 0.009 & 0.780 & 0.696 & 0.034 \\

\hline 

U-Net v2 (ours) & \textbf{92.8} & \textbf{88.0} & \textbf{0.019}& \textbf{94.4} & \textbf{89.6} & \textbf{0.006} & \textbf{81.2} & \textbf{73.1} & \textbf{0.030}

% our method & & & & \\
\end{tabular}

\caption{Experimental comparison with state-of-the-art methods on the Kvasir-SEG, ClinicDB, and ColonDB datasets.}

\label{tab:polyp_1}
\end{table*}



==> tables/polyp_2.tex <==
\begin{table*}[h!]
\centering
\small
\begin{tabular}{c|ccccccccc}

\multirow{2}{*}{method} & \multicolumn{3}{c}{ETIS} & \multicolumn{3}{c}{Endoscene} \\

\cline{2-7}

& DSC (\%)& mIoU (\%)  & MAE & DSC (\%) &mIoU (\%) &  MAE  \\

\hline 

U-Net~\cite{ronneberger2015u} & 39.8 & 33.5 & 0.036 & 71.0 & 62.7 & 0.022 \\

UNet++~\cite{zhou2018unet++} & 40.1 & 34.4 & 0.035 & 70.7 & 62.4 & 0.018\\

PraNet~\cite{fan2020pranet} & 62.8 & 56.7 & 0.031 & 87.1 & 79.7 & 0.010\\

SANet~\cite{wei2021shallow} & 75.0 & 65.4 & 0.015 & 88.8 & 81.5 & 0.008\\

Polyp-PVT~\cite{dong2021polyp} & 78.7 & \textbf{70.6} & \textbf{0.013} & \textbf{90.0} & \textbf{83.3} & \textbf{0.007}\\

% UNet (PVT)~\cite{ronneberger2015u} & 0.780 & 0.709& 0.016 & 0.885 & 0.816 & 0.009\\
% UNet++ (PVT)~\cite{ronneberger2015u} & 0.759 & 0.691& 0.022 & 0.879 & 0.804 & 0.009\\

\hline

U-Net v2 (ours) & \textbf{79.0} & {70.5} & \textbf{0.013} & 89.7 & 83.1 & \textbf{0.007}
\end{tabular}

\caption{Experimental comparison with state-of-the-art methods on the ETIS and Endoscene datasets.}

\label{tab:polyp_2}
\end{table*}

==> tables/polyp_ablation.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{c|cccc}
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{kavans} & \multicolumn{2}{c}{ClinicDB} \\
\cline{2-5}
    & mIoU (\%) & DSC (\%) & mIoU (\%) & DSC (\%) \\
\hline 
nnU-Net & & & & \\

Our method & & & &
\end{tabular}
\caption{Experimental comparison with state-of-the art methods on the polyp datasets.}
\label{tab:polyp_ablation}
\end{table*}

==> tables/polyp_old.tex <==
\begin{table*}[!h]
\centering

\begin{tabular}{c|cccccccccccc}

\multirow{2}{*}{Method} & \multicolumn{3}{c}{Kvasir-SEG} & \multicolumn{3}{c}{ClinicDB} & \multicolumn{3}{c}{ColonDB}\\

\cline{2-10}

& DSC (\%) & mIoU (\%)  & MAE & DSC (\%) &mIoU (\%)  & MAE & DSC (\%) & mIoU (\%) &  MAE \\

\hline 

U-Net~\cite{ronneberger2015u}  & 81.8 & 74.6 & 0.055 & 82.3 & 75.5 & 0.019 & 51.2 & 44.4 & 0.061 \\

UNet++~\cite{zhou2018unet++} & 82.1 & 74.3 & 0.048 & 79.4 & 72.9 & 0.022 & 48.3 & 41.0 & 0.064\\

PraNet~\cite{fan2020pranet} & 89.8 & 84.0 & 0.030 & 89.9 & 84.9 & 0.009 & 71.2 & 64.0 & 0.043 \\

SANet~\cite{wei2021shallow} & 90.4 & 84.7 & 0.028 & 91.6 & 85.9 & 0.012 & 75.3 & 67.0 & 0.043\\

Polyp-PVT~\cite{dong2021polyp} & 91.7 & 86.4 & 0.023 & 93.7 & 88.9 & \textbf{0.006} & 80.8 & 72.7 & 0.031\\

% U-Net (PVT)~\cite{ronneberger2015u} & 0.925 & 0.875 & 0.023 & 0.936 & 0.888 & 0.007 & 0.792 & 0.715 & 0.030 \\

% UNet++ (PVT)~\cite{zhou2018unet++} & 0.928 & 0.879 & 0.020 & 0.933 & 0.885 & 0.009 & 0.780 & 0.696 & 0.034 \\

\hline 

U-Net v2 (ours) & \textbf{92.8} & \textbf{88.0} & \textbf{0.019}& \textbf{94.4} & \textbf{89.6} & \textbf{0.006} & \textbf{81.2} & \textbf{73.1} & \textbf{0.030}

% our method & & & & \\
\end{tabular}

\caption{Experimental comparison with state-of-the-art methods on the Kvasir-SEG, ClinicDB, and ColonDB datasets.}

\label{tab:polyp_1}
\end{table*}



==> tables/retina_ablation.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{c|cccc}
\multirow{2}{*}{Method} & \multicolumn{2}{c}{ISIC 2017} & \multicolumn{2}{c}{ISIC 2018} \\
\cline{2-5}
    & mIoU (\%) & DSC (\%) & mIoU (\%) & DSC (\%) \\
\hline 
nnU-Net & & & & \\

Our method & & & &
\end{tabular}
\caption{Experimental comparison with state-of-the art methods on the retina fluid datasets.}
\label{tab:retina_ablation}
\end{table*}

==> tables/retinal.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{c|cccccccc}
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Cirrus} & \multicolumn{2}{c}{Spectralis} & \multicolumn{2}{c}{Topcon} & \multicolumn{2}{c}{Iowa dataset}\\
\cline{2-9}
    & DSC (\%) & AVD & DSC (\%) & AVD & DSC (\%) & AVD & DSC (\%) & AVD \\
\hline 
DeepLabv3+ \\
U-Net \\
Att-UNet \\
CPF-Net \\
Curvature \\
MsTGANet \\
nnU-Net & & & & \\
\hline
Our method & & & &
\end{tabular}
\caption{Experimental comparison with state-of-the art methods on the retina fluid datasets.}
\label{tab:retina}
\end{table*}
